Bridging Distribution Gaps in Time Series Foundation Model Pretraining with Prototype-Guided Normalization

Foundation models have achieved remarkable success across diverse machine-learning domains through large-scale pretraining on large, diverse datasets. However, pretraining on such datasets introduces significant challenges due to substantial mismatches in data distributions, a problem particularly pronounced with time series data. In this paper, we tackle this issue by proposing a domain-aware adaptive normalization strategy within the Transformer architecture. Specifically, we replace the traditional LayerNorm with a prototype-guided dynamic normalization mechanism (ProtoNorm), where learned prototypes encapsulate distinct data distributions, and sample-to-prototype affinity determines the appropriate normalization layer. This mechanism effectively captures the heterogeneity of time series characteristics, aligning pretrained representations with downstream tasks. Through comprehensive empirical evaluation, we demonstrate that our method significantly outperforms conventional pretraining techniques across both classification and forecasting tasks, while effectively mitigating the adverse effects of distribution shifts during pretraining. Incorporating ProtoNorm is as simple as replacing a single line of code. Extensive experiments on diverse real-world time series benchmarks validate the robustness and generalizability of our approach, advancing the development of more versatile time series foundation models.

==> tables/Moirai_results/ood_lsf_MAE_results.tex <==
\begin{table*}[htbp]
\centering
\caption{Comparison of MAE across Different Models and Prediction Lengths on long sequence forecasting experiments}
\begin{tabular}{l|c|ccccc}
\hline
Dataset & Length & MOIRAI$_{\text{Small}}$ & \texttt{ProtoN4-FM} & \texttt{ProtoN8-FM} & \texttt{ProtoN16-FM} & \texttt{ProtoN32-FM} \\
\hline
\multirow{5}{*}{ETTh1} 
& 96 & 0.4033 & 0.4044 & 0.4026 & \textbf{0.4007} & 0.4029 \\
& 192 & 0.4209 & 0.4237 & 0.4225 & \textbf{0.4189} & 0.4212 \\
& 336 & 0.4314 & 0.4347 & 0.4339 & \textbf{0.4282} & 0.4331 \\
& 720 & 0.4473 & 0.4579 & 0.4522 & \textbf{0.4463} & 0.4532 \\
\rowcolor{gray!20}
& Avg & 0.4257 & 0.4302 & 0.4278 & \textbf{0.4235} & 0.4276 \\
\hline
\multirow{5}{*}{ETTh2} 
& 96 & 0.3329 & 0.3323 & 0.3352 & \textbf{0.3309} & 0.3348 \\
& 192 & 0.3734 & \textbf{0.3707} & 0.3734 & 0.3712 & 0.3756 \\
& 336 & 0.3922 & \textbf{0.3864} & 0.3890 & 0.3903 & 0.3933 \\
& 720 & 0.4110 & \textbf{0.4050} & 0.4081 & 0.4064 & 0.4096 \\
\rowcolor{gray!20}
& Avg & 0.3774 & \textbf{0.3736} & 0.3764 & 0.3747 & 0.3783 \\
\hline
\multirow{5}{*}{ETTm1}
& 96 & 0.3681 & 0.3700 & \textbf{0.3667} & 0.3780 & 0.3775 \\
& 192 & \textbf{0.3820} & 0.3870 & 0.3839 & 0.3995 & 0.3916 \\
& 336 & \textbf{0.3962} & 0.4023 & 0.3971 & 0.4164 & 0.4037 \\
& 720 & 0.4187 & 0.4236 & \textbf{0.4177} & 0.4452 & 0.4243 \\
\rowcolor{gray!20}
& Avg & \textbf{0.3913} & 0.3957 & 0.3914 & 0.4098 & 0.3993 \\
\hline
\multirow{5}{*}{ETTm2}
& 96 & 0.2869 & \textbf{0.2782} & 0.2833 & 0.2783 & 0.2865 \\
& 192 & 0.3264 & 0.3184 & 0.3222 & \textbf{0.3155} & 0.3251 \\
& 336 & 0.3596 & 0.3547 & 0.3555 & \textbf{0.3501} & 0.3568 \\
& 720 & 0.4063 & 0.4028 & 0.4038 & \textbf{0.4005} & 0.4048 \\
\rowcolor{gray!20}
& Avg & 0.3448 & 0.3385 & 0.3412 & \textbf{0.3361} & 0.3433 \\
\hline
\multirow{5}{*}{Electricity}
& 96 & 0.2868 & 0.2806 & 0.2875 & \textbf{0.2794} & 0.2828 \\
& 192 & 0.2989 & 0.2924 & 0.3002 & \textbf{0.2910} & 0.2937 \\
& 336 & 0.3112 & 0.3054 & 0.3124 & \textbf{0.3049} & 0.3059 \\
& 720 & 0.3362 & \textbf{0.3305} & 0.3381 & 0.3314 & 0.3314 \\
\rowcolor{gray!20}
& Avg & 0.3083 & 0.3022 & 0.3096 & \textbf{0.3017} & 0.3035 \\
\hline
\multirow{5}{*}{Weather}
& 96 & 0.2126 & 0.2091 & 0.2086 & \textbf{0.2057} & 0.2094 \\
& 192 & 0.2493 & \textbf{0.2449} & 0.2471 & 0.2478 & 0.2465 \\
& 336 & 0.2817 & \textbf{0.2786} & 0.2808 & 0.2832 & 0.2809 \\
& 720 & \textbf{0.3210} & 0.3238 & 0.3238 & 0.3289 & 0.3251 \\
\rowcolor{gray!20}
& Avg & 0.2662 & \textbf{0.2641} & 0.2651 & 0.2664 & 0.2655 \\
\hline
\end{tabular}
\end{table*}


==> tables/Moirai_results/ood_lsf_MSE_results.tex <==
\begin{table*}[htbp]
\centering
\caption{Comparison of MSE across Different Models and Prediction Lengths on long sequence forecasting experiments}
\begin{tabular}{l|c|ccccc}
\hline
Dataset & Length & MOIRAI$_{\text{Small}}$ & \texttt{ProtoN4-FM} & \texttt{ProtoN8-FM} & \texttt{ProtoN16-FM} & \texttt{ProtoN32-FM} \\
\hline
\multirow{5}{*}{ETTh1} 
& 96 & 0.3756 & 0.3744 & \textbf{0.3698} & 0.3797 & 0.3728 \\
& 192 & 0.4000 & 0.4006 & \textbf{0.3953} & 0.4067 & 0.3975 \\
& 336 & 0.4112 & 0.4154 & \textbf{0.4097} & 0.4165 & 0.4128 \\
& 720 & \textbf{0.4170} & 0.4377 & 0.4252 & 0.4203 & 0.4242 \\
\rowcolor{gray!20}
& Avg & 0.4010 & 0.4070 & \textbf{0.4000} & 0.4058 & 0.4018 \\
\hline
\multirow{5}{*}{ETTh2} 
& 96 & 0.2868 & 0.2842 & 0.2920 & \textbf{0.2841} & 0.2873 \\
& 192 & 0.3487 & \textbf{0.3427} & 0.3512 & 0.3453 & 0.3515 \\
& 336 & 0.3709 & \textbf{0.3625} & 0.3696 & 0.3717 & 0.3769 \\
& 720 & 0.3848 & \textbf{0.3719} & 0.3817 & 0.3796 & 0.3812 \\
\rowcolor{gray!20}
& Avg & 0.3478 & \textbf{0.3403} & 0.3486 & 0.3452 & 0.3492 \\
\hline
\multirow{5}{*}{ETTm1}
& 96 & 0.3698 & \textbf{0.3632} & 0.3645 & 0.4090 & 0.3819 \\
& 192 & \textbf{0.3785} & 0.3849 & 0.3814 & 0.4514 & 0.3958 \\
& 336 & 0.3955 & 0.4074 & \textbf{0.3941} & 0.4837 & 0.4068 \\
& 720 & 0.4261 & 0.4415 & \textbf{0.4252} & 0.5311 & 0.4315 \\
\rowcolor{gray!20}
& Avg & 0.3925 & 0.3993 & \textbf{0.3913} & 0.4688 & 0.4040 \\
\hline
\multirow{5}{*}{ETTm2}
& 96 & 0.2135 & \textbf{0.2014} & 0.2094 & 0.2041 & 0.2096 \\
& 192 & 0.2768 & 0.2629 & 0.2711 & \textbf{0.2621} & 0.2707 \\
& 336 & 0.3304 & 0.3183 & 0.3252 & \textbf{0.3178} & 0.3228 \\
& 720 & 0.4047 & \textbf{0.3969} & 0.4017 & 0.4002 & 0.3975 \\
\rowcolor{gray!20}
& Avg & 0.3064 & \textbf{0.2949} & 0.3019 & 0.2961 & 0.3002 \\
\hline
\multirow{5}{*}{Electricity}
& 96 & 0.1948 & 0.1878 & 0.1959 & \textbf{0.1861} & 0.1911 \\
& 192 & 0.2106 & 0.2026 & 0.2119 & \textbf{0.2009} & 0.2051 \\
& 336 & 0.2247 & 0.2180 & 0.2260 & \textbf{0.2172} & 0.2190 \\
& 720 & 0.2582 & 0.2519 & 0.2595 & \textbf{0.2516} & 0.2522 \\
\rowcolor{gray!20}
& Avg & 0.2221 & 0.2151 & 0.2233 & \textbf{0.2139} & 0.2169 \\
\hline
\multirow{5}{*}{Weather}
& 96 & 0.1760 & 0.1741 & 0.1734 & \textbf{0.1714} & 0.1758 \\
& 192 & 0.2172 & \textbf{0.2137} & 0.2158 & 0.2175 & 0.2156 \\
& 336 & 0.2626 & \textbf{0.2604} & 0.2634 & 0.2652 & 0.2631 \\
& 720 & \textbf{0.3189} & 0.3292 & 0.3290 & 0.3318 & 0.3300 \\
\rowcolor{gray!20}
& Avg & \textbf{0.2437} & 0.2444 & 0.2454 & 0.2465 & 0.2461 \\
\hline
\end{tabular}
\end{table*}


==> tables/datasets/FD_intro.tex <==


% == Datasets description table ==
\begin{table}[!tbh]
\centering
\caption{A description of characteristics of the datasets on FD task used in our experiments.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1.2mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{l|ccccc}
\toprule
Dataset & \# Train  & \# Test & Length & \# Channel & \# Class \\ \midrule

IMS & 42492  & 14164 & 20480 & 1 & 4  \\ 
UO & 42184 & 14061 & 2000000 & 2 & 3  \\ 
PU & 163296 & 54432 & 249600 & 1 & 14  \\ 
\bottomrule
\end{NiceTabular}
}}
\label{table:fd_datasets}
\end{table}

==> tables/datasets/HAR_intro.tex <==
% == Datasets description table ==
\begin{table}[!tbh]
\centering
\caption{A description of characteristics of the datasets on HAR task used in our experiments.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1.2mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{l|ccccc}
\toprule
Dataset & \# Train  & \# Test & Length & \# Channel & \# Class \\ \midrule

HHAR & 10233  & 4436 & 128 & 3 & 6  \\ 
SKODA & 2919 & 974 & 177 & 5 & 10  \\ 
UCIHAR & 5881 & 2947 & 128 & 9 & 6  \\ 
USCHAD & 2992 & 1008 & 500 & 6 & 12  \\ 
WISDM & 6309 & 2104 & 100 & 3 & 6  \\ 
\bottomrule
\end{NiceTabular}
}}
\label{table:har_datasets}
\end{table}

==> tables/datasets/otherPHM_intro.tex <==
% == Datasets description table ==
\begin{table}[!tbh]
\centering
\caption{A description of characteristics of the datasets on other related PHM datasets.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{0.5mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{l|ccccc}
\toprule
Dataset & \# Train  & \# Val & Length & \# Channel & Sample Rating \\ \midrule

CWRU & 280  & 2201 & 120000 & 2 & 12kHz  \\ 
FEMTO & 11794 & 11934 & 2560 & 2 & 25.6kHz  \\ 
XJTUSY & 191040 & 202912 & 32768 & 2 & 25.6kHz  \\ 
\bottomrule
\end{NiceTabular}
}}
\label{table:other_phm_datasets}
\end{table}

==> tables/main/out_domain/generalization_results.tex <==

\begin{table}[ht]
  \begin{minipage}[h]{0.45\hsize}   
  \renewcommand\arraystretch{1.0} 
  \centering
  
  \caption{Detailed results of generalization performance comparison of vanilla pretraining method and \abb on FD Tasks. We calculate the Accuracy and F1-score (\%) for each dataset. The best average performance results are \textbf{bolded}.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{@{}l|cc|cc@{}} 
\toprule 
\multirow{2}*{Datasets} & \multicolumn{2}{c|}{Accuracy} & \multicolumn{2}{c}{Macro-F1} \\ \cline{2-5}
 & Vanilla & \abb & Vanilla & \abb \\ \midrule
IMS   & {50.10} & \textbf{54.66} & {42.69} & \textbf{45.12} \\
UO    & {68.23} & \textbf{72.88} & {67.64} & \textbf{72.40} \\
PU    & {07.33}  & \textbf{12.65} & {01.47}  & \textbf{05.58}  \\ \midrule \rowcolor{gray!20}
Average & {41.89} & \textbf{46.73} & {37.27} & \textbf{41.03} \\
\bottomrule
\end{NiceTabular}
}}
\label{table:phm_outdomain}
    
  \end{minipage}
  \hspace{0.35cm}
  \begin{minipage}[h]{0.45\hsize}
  \centering        
  \renewcommand\arraystretch{1.0} 

\caption{Detailed results of generalization performance comparison of vanilla pretraining method and \abb on HAR Tasks. We calculate the Accuracy and F1-score (\%) for each dataset. The best average performance results are \textbf{bolded}.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{@{}l|cc||cc@{}} 
\toprule 
\multirow{2}*{Datasets} & \multicolumn{2}{c|}{Accuracy} & \multicolumn{2}{c}{Macro-F1} \\ \cline{2-5}
 & Vanilla & \abb & Vanilla & \abb \\ \midrule
HHAR   & {70.18} & \textbf{70.51} & {62.18} & \textbf{62.64} \\
SKODA  & {22.45} & \textbf{23.58} & {15.09} & \textbf{15.57} \\
UCHIAR & {57.64} & \textbf{58.49} & {45.38} & \textbf{46.29} \\
USCHAD & {31.75} & \textbf{35.65} & {19.49} & \textbf{23.30} \\ 
WISDM  & {56.86} & \textbf{57.37} & {39.45} & \textbf{39.65} \\ \midrule \rowcolor{gray!20}
Average & {47.78} & \textbf{49.12} & {36.32} & \textbf{37.49} \\
\bottomrule
\end{NiceTabular}
}}
\label{table:har_outdomain}
    
  \end{minipage}
  \end{table}

==> tables/main/out_domain/main_out_domain_har_results.tex <==
\begin{table*}[h]
\centering
\caption{Detailed results of generalization performance comparison of vanilla pretraining method and \abb on HAR Task. We calculate the Accuracy and F1-score (\%) for each dataset. The best average performance results are \textbf{bolded}.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{@{}l|cc||cc@{}} 
\toprule 
\multirow{2}*{Datasets} & \multicolumn{2}{c|}{Accuracy} & \multicolumn{2}{c}{Macro-F1} \\ \cline{2-5}
 & Vanilla & \abb & Vanilla & \abb \\ \midrule
HHAR   & 70.18 & \textbf{70.51} & 62.18 & \textbf{62.64} \\
SKODA  & 22.45 & \textbf{23.58} & 15.09 & \textbf{15.57} \\
UCHIAR & 57.64 & \textbf{58.49} & 45.38 & \textbf{46.29} \\
USCHAD & 31.75 & \textbf{35.65} & 19.49 & \textbf{23.30} \\ 
WISDM  & 56.86 & \textbf{57.37} & 39.45 & \textbf{39.65} \\ \midrule \rowcolor{gray!20}
Average & 47.78 & \textbf{49.12} & 36.32 & \textbf{37.49} \\
\bottomrule
\end{NiceTabular}
}}
\label{table:har_outdomain}
\end{table*}


==> tables/main/out_domain/main_out_domain_phm_results.tex <==
% \begin{table*}[h]
% \centering
% {\fontsize{9}{11}\selectfont
% \setlength{\tabcolsep}{2.5mm}{
% \renewcommand\arraystretch{0.9}
% \begin{NiceTabular}{@{}l|cc|cc|cc|cc@{}} 
% \toprule 
% \multirow{2}*{Datasets} & \multicolumn{2}{c|}{Sup} & \multicolumn{2}{c|}{Individual} & \multicolumn{2}{c|}{Vanilla} & \multicolumn{2}{c}{DA-MoLN} \\ \cline{2-9}
%  & Acc & MF1 & Acc & MF1 & Acc & MF1 & Acc & MF1 \\ \midrule
% IMS & 54.22 & 47.84 & 59.48 & 57.79 & 50.10 & 42.69 & 54.66 & 45.12 \\
% UO & 49.32 & 48.20 & 50.62 & 49.33 & 68.23 & 67.64 & 72.88 & 72.40 \\
% PU & 48.19 & 44.61 & 58.42 & 54.98 & 7.33 & 1.47 & 12.65 & 5.58 \\ \midrule
% Average & 50.58 & 46.88 & 56.17 & 54.03 & 41.89 & 37.27 & 46.73 & 41.03 \\
% \bottomrule
% \end{NiceTabular}
% }}
% \caption{Out-domain performance comparison of various methods on PHM Tasks.}
% \label{table:phm_outdomain}
% \end{table*}

% \begin{table*}[h]
% \centering
% {\fontsize{9}{11}\selectfont
% \setlength{\tabcolsep}{2.5mm}{
% \renewcommand\arraystretch{0.9}
% \begin{NiceTabular}{@{}l|cc|cc|cc|cc@{}} 
% \toprule 
% \multirow{2}*{Datasets} & \multicolumn{2}{c|}{Sup} & \multicolumn{2}{c|}{Individual} & \multicolumn{2}{c|}{Vanilla} & \multicolumn{2}{c}{DA-MoLN} \\ \cline{2-9}
%  & Acc & MF1 & Acc & MF1 & Acc & MF1 & Acc & MF1 \\ \midrule
% IMS & 54.22 & 47.84 & 59.48 & 57.79 & 50.10 & 42.69 & 54.66 & 45.12 \\
% UO & 49.32 & 48.20 & 50.62 & 49.33 & 68.23 & 67.64 & 72.88 & 72.40 \\
% PU & 48.19 & 44.61 & 58.42 & 54.98 & 7.33 & 1.47 & 12.65 & 5.58 \\ \midrule
% Average & 50.58 & 46.88 & 56.17 & 54.03 & 41.89 & 37.27 & 46.73 & 41.03 \\
% \bottomrule
% \end{NiceTabular}
% }}
% \caption{Out-domain performance comparison of various methods on PHM Tasks.}
% \label{table:phm_outdomain}
% \end{table*}

\begin{table*}[h]
\centering
\caption{Detailed results of generalization performance comparison of vanilla pretraining method and \abb on FD Task. We calculate the Accuracy and F1-score (\%) for each dataset. The best average performance results are \textbf{bolded}.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{@{}l|cc|cc@{}} 
\toprule 
\multirow{2}*{Datasets} & \multicolumn{2}{c|}{Accuracy} & \multicolumn{2}{c}{Macro-F1} \\ \cline{2-5}
 & Vanilla & \abb & Vanilla & \abb \\ \midrule
IMS   & 50.10 & \textbf{54.66} & 42.69 & \textbf{45.12} \\
UO    & 68.23 & \textbf{72.88} & 67.64 & \textbf{72.40} \\
PU    & 07.33  & \textbf{12.65} & 01.47  & \textbf{5.58}  \\ \midrule \rowcolor{gray!20}
Average & 41.89 & \textbf{46.73} & 37.27 & \textbf{41.03} \\
\bottomrule
\end{NiceTabular}
}}
\label{table:phm_outdomain}
\end{table*}





==> tables/parameter_analysis/num_experts.tex <==
\begin{table*}[h]
\centering
\caption{Performance comparison using different number of LayerNorms accross various datasets on both FD and HAR tasks. We calculate the Accuracy and F1-score (\%) for each dataset. Best average performance results are \textbf{bolded}.}
{\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2.5mm}{
\renewcommand\arraystretch{1.0}
\begin{NiceTabular}{@{}l|cccc||cccc@{}} 
\toprule 
\multirow{2}*{Datasets} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c}{Macro-F1} \\ \cline{2-9}
 & $2$ & $3$ & $4$ & $\#D$ & $2$ & $3$ & $4$ & $\#D$ \\ \midrule
IMS  & 78.14 & 78.78 & 78.33  & 77.23 & 71.92 & 73.03 & 71.51 & 70.40 \\
UO   & 66.83 & 68.56 & 67.60  & 68.48 & 66.10 & 67.93 & 66.77 & 67.72 \\ 
PU   & 63.38 & 63.65 & 63.42  & 64.91 & 60.08 & 60.43 & 60.14 & 61.61 \\ \rowcolor{gray!20}
Average & 69.45 & \textbf{70.33} & 69.78 & 70.21 & 66.03 & \textbf{67.80} & 66.81 & 66.58 \\ \midrule \midrule
HHAR  & 72.09 & 72.29 & 72.22  & 72.43 & 64.12 & 64.11 & 64.21 & 64.36 \\
SKODA & 26.01 & 24.26 & 23.48  & 25.56 & 16.27 & 15.93 & 15.50 & 16.94 \\ 
UCIHAR & 59.24 & 59.11 & 59.29 & 59.38 & 46.70 & 46.72 & 46.58 & 46.69 \\ 
USCHAD & 36.24 & 35.78 & 36.01 & 36.64 & 23.43 & 23.23 & 23.34 & 23.86 \\ 
WISDM  & 63.48 & 60.85 & 62.69 & 61.25 & 43.70 & 42.56 & 42.87 & 42.67 \\ \rowcolor{gray!20}
Average & 51.81 & 50.46 & 50.74 & \textbf{51.85} & 38.44 & 38.11 & 38.10 & \textbf{38.50} \\
\bottomrule
\end{NiceTabular}
}}
\label{table:num_experts}
\end{table*}



















